Rhino: An Autonomous Robot for Mapping Underground Mine Environments

There are many benefits for exploring and exploiting underground mines, but there are also significant risks and challenges. One such risk is the potential for accidents caused by the collapse of the pillars, and roofs which can be mitigated through inspections. However, these inspections can be costly and may put the safety of the inspectors at risk. To address this issue, this work presents Rhino, an autonomous robot that can navigate underground mine environments and generate 3D maps. These generated maps will allow mine workers to proactively respond to potential hazards and prevent accidents. The system being developed is a skid-steer, four-wheeled unmanned ground vehicle (UGV) that uses a LiDAR and IMU to perform long-duration autonomous navigation and generation of maps through a LIO-SAM framework. The system has been tested in different environments and terrains to ensure its robustness and ability to operate for extended periods of time while also generating 3D maps.

==> reviews.tex <==
-------------------------------------------------------
Senior Editor: 1
Comments to the Author:
%The TE obtained three reviews of this submission. Overall the Reviewers found that the novelty and contribution of the work to the field is limited and minor, and the writing is unclear and needs to be significantly improved. All the reviewers don't see that the paper can be improved quickly for this FS given the short period of time and the issues that need to be addressed.

%I concurred with the TE's evaluation. Given these critical concerns and the tight revision time for the FS, I cannot recommend the paper for further consideration. However, both the TE and I believe that the paper is a good fit and candidate to the AIM 2023, and we would strongly suggest the authors to keep their submission for the AIM consideration, including the presentation-only option. The authors are referred to the AIM 2023 website for detail.



Technical Editor: 2
Comments to the Author:
%The paper presents the development of an autonomous robot for surveying an area. There is rich information regarding this subject and a critical review of existing literature is needed. Justifications for the proposed design should be provided.  There is a lack of novelty in both hardware and software. Innovative contributions to knowledge should be clearly articulated. The presentation of the paper is of a poor quality too. For instance, Figure 3 has many blank boxes, which indicates it is not completed.

Chris: There was an error with the compiling, apparently this is a recurrent problem on TMECH template, because I reviewd paper like this that I thought was poor quality as well, but it is not our fault. The ieee conference template should work well

--------------------------------------------------------
REVIEWERS' SUGGESTIONS:

Reviewer: 1
WHAT ARE THE CONTRIBUTIONS OF THIS PAPER: In this paper, authors present Rhino, a robotic system for monitoring underground stone mines. It is an unmanned ground vehicle equipped with various sensors and electronics. In practice, the system is able to autonomously traverse difficult terrain for 6 continuous hours outdoors.

Reviewer: 2
WHAT ARE THE CONTRIBUTIONS OF THIS PAPER: It's very hard to say. The Reviewer couldn't find any significant contribution from the manuscript.

Reviewer: 3
WHAT ARE THE CONTRIBUTIONS OF THIS PAPER: There is no real contribution as far as I could understand.

Reviewer: 1
WHAT ARE SOME WAYS IN WHICH THE PAPER COULD BE IMPROVED: Major Issue:
After reading the entire article, I felt like I read an abbreviated engineering report. The author has designed a wheeled robot called "Rhino", which is mediocre in both the hardware design and software parts. The tethered drone I was expecting were not mentioned later in the paper. Overall, this paper is an abbreviated engineering summary but lacks innovation.
Minor Issues:
1.      Figures 3 and 4 both have parts that are not fully displayed.
2.      Since the localization method uses the advanced and mature method LIO-SAM, the subsequent experiments to verify the localization accuracy lack significance.

Reviewer: 2
WHAT ARE SOME WAYS IN WHICH THE PAPER COULD BE IMPROVED: If this work was reported five years ago, it might be worth a journal article, assuming some revisions. However, as pointed out multiple times by the authors in the paper, the recent advances in subterranean navigation and mapping made the authors' work obsolete. Integrating a mobile robot, navigating through an underground mine, and getting a map of the mine can no longer be regarded as an academic contribution. Making a system with a longer operation time than others is not enough at all. Authors should provide evidences about why their approach is better than others through more comparative studies.

Reviewer: 3
WHAT ARE SOME WAYS IN WHICH THE PAPER COULD BE IMPROVED: The paper needs much improvement and a clear contribution. Just building a robot is not a contribution.

Reviewer: 1

Comments to the Author
Underground mine autonomous exploration is a very good topic, but need to explore more innovative points.

Reviewer: 2

Comments to the Author
It was pretty shocking to the Reviewer that the paper was submitted with incomplete system diagrams (Figs 3 and 4). The report of the experiments is insufficient and provides no value to the work. Please think about what changes the authors made on top of existing algorithms and show how those changes improved the system's performance.

Reviewer: 3

Comments to the Author
This work presents Rhino, an autonomous robot that can navigate underground mine environments and generate 3D maps. These generated maps will allow mine workers to proactively respond to potential hazards and prevent accidents. The system being developed is a skid-steer, four-wheeled unmanned ground vehicle (UGV) that uses a LiDAR and IMU to perform long-duration autonomous navigation and generation of maps through a LIO-SAM framework. Although the research problem is interesting, I do not recommend publication due to the following reasons:

There is no contribution.

Figure 3 is weird. There is nothing written.

The real robot in this work does not have any drone base or drone.

All the algorithms used are not novel, just an application.

SOTA is very bad. Too many arXiv manuscripts, old papers, and only 12 relevant new ones (>=2017) out of 37.



TODO: add something with the drone
      fix typos
      remove localization results maybe, and add new test results
    
